You Cannot Fix What You Cannot Find! An Investigation of Fault Localization Bias in Benchmarking Automated Program Repair Systems

Properly benchmarking Automated Program Repair (APR) systems should contribute to the development and adoption of the research outputs by practitioners. To that end, the research community must ensure that it reaches significant milestones by reliably comparing state-of-the-art tools for a better understanding of their strengths and weaknesses. In this work, we identify and investigate a practical bias caused by the fault localization (FL) step in a repair pipeline. We propose to highlight the different fault localization configurations used in the literature, and their impact on APR systems when applied to the Defects4J benchmark. Then, we explore the performance variations that can be achieved by `tweaking' the FL step. Eventually, we expect to create a new momentum for (1) full disclosure of APR experimental procedures with respect to FL, (2) realistic expectations of repairing bugs in Defects4J, as well as (3) reliable performance comparison among the state-of-the-art APR systems, and against the baseline performance results of our thoroughly assessed kPAR repair tool. Our main findings include: (a) only a subset of Defects4J bugs can be currently localized by commonly-used FL techniques; (b) current practice of comparing state-of-the-art APR systems (i.e., counting the number of fixed bugs) is potentially misleading due to the bias of FL configurations; and (c) APR authors do not properly qualify their performance achievement with respect to the different tuning parameters implemented in APR systems.

==> relatedwork.tex <==
\section{Related Work}
\label{sec:relatedWork}

==> table/aprPart1 <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c?c|c|c?c|c|c?c|c|c?c|c|c?c|c|c?c|c|c?c|c|c|}
\hline
&	&	&	&	&	&	&	&	&	&	&	&	&\multicolumn{3}{l?}{{Tarantula}} & \multicolumn{3}{l?}{{Ochiai}} & \multicolumn{3}{l?}{{Dstar2}} & \multicolumn{3}{l?}{{Barinel}} & \multicolumn{3}{l?}{{Opt2}} & \multicolumn{3}{l?}{{Muse}} & \multicolumn{3}{l|}{{Jaccard}} \\
\hline
\rotatebox[origin=l]{0}{Project} & \rotatebox[origin=l]{90}{SimFix} & \rotatebox[origin=l]{90}{CapGen} & \rotatebox[origin=l]{90}{SketchFix} & \rotatebox[origin=l]{90}{JAID} & \rotatebox[origin=l]{90}{ssFix} & \rotatebox[origin=l]{90}{ACS} & \rotatebox[origin=l]{90}{ELIXIR} & \rotatebox[origin=l]{90}{HDRepair} & \rotatebox[origin=l]{90}{jGenProg} & \rotatebox[origin=l]{90}{jKali} & \rotatebox[origin=l]{90}{jMutRepair} & \rotatebox[origin=l]{90}{Nopol}	 & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                    & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                  & \rotatebox[origin=l]{90}{Line}                 & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                   & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                 & \rotatebox[origin=l]{90}{File}                    & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method} \\
       
\hline
Chart-1	    		 & \cmark & \cmark & \cmark & (\cmark) & \cmark &	& \cmark & \xmark & \xmark & \xmark & \cmark & 			& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-3	    		 & \cmark &	&	&	&	&	& \xmark &	& \xmark &	&	& \xmark											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-5	    		 &	&	&	&	&	&	&	&	& \xmark & \xmark &	& \cmark												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-7	    		 & \cmark &	&	&	&	&	&	&	& \xmark &	& \xmark & 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-8	    		 &	& \cmark & \cmark &	&	&	& \cmark & \xmark &	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-9	    		 &	&	& \cmark & (\cmark) &	&	& \cmark &	&	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-11			 &	& \cmark & \cmark &	&	&	& \cmark &	&	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-12			 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-13			 &	&	& \xmark &	&	&	& \xmark &	& \xmark & \xmark &	& \xmark										& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-14			 & \xmark &	&	&	&	& \cmark &	&	&	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-15			 &	&	&	&	&	&	&	&	& \xmark & \xmark &	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \rmark &     \rmark &      \cmark &      \cmark &      \cmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Chart-17			 &	&	&	&	&	&	& \xmark &	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-18			 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-19			 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-20			 & \cmark &	& \cmark &	& \cmark &	&	&	&	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-21			 &	&	&	&	&	&	&	&	&	&	&	& \xmark														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-22			 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-24			 &	& \cmark & \cmark & \cmark & \cmark &	&	&	&	&	&	& 											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Chart-25			 &	&	&	&	&	&	&	&	& \xmark & \xmark & \xmark & \xmark											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \rmark &     \rmark &      \cmark &      \cmark &      \cmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Chart-26			 &	&	& \xmark & \cmark &	&	&	&	&	& \xmark & \xmark & \xmark										& \rmark &        \rmark &        \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &      \rmark &      \rmark &      \rmark &   \rmark &   \rmark &   \rmark &   \rmark &   \rmark &   \rmark &      \rmark &      \rmark &      \rmark \\
\hline
Closure-5			 &	&	&	& \xmark &	&	&	&	&	&	&	& 															& \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Closure-10			 &	&	&	&	&	&	&	& \xmark &	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-14			 & \cmark &	& \cmark &	& \cmark &	&	& \xmark &	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-18			 &	&	&	& \cmark &	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-31			 &	&	&	& (\cmark) &	&	&	&	&	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-33			 &	&	&	& \cmark &	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-40			 &	&	&	& \cmark &	&	&	&	&	&	&	& 															& \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Closure-51			 &	&	&	&	&	&	&	& \xmark &	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-57			 & \cmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-62			 & \cmark &	& \cmark & (\cmark) &	&	&	& \xmark &	&	&	& 											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-63			 & \cmark &	&	& (\cmark) &	&	&	&	&	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-70			 &	&	& \xmark & \cmark &	&	&	& \xmark &	&	&	& 													& \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Closure-73			 & \cmark &	& \xmark & \cmark &	&	&	& \xmark &	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-79			 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-106			 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-115			 & \cmark &	&	&	& \cmark &	&	&	&	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-125			 &	&	&	& \xmark &	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Closure-126			 &	&	& \cmark & (\cmark) &	&	&	& \xmark &	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
\hline
Lang-6	    		 &	& \cmark & \cmark &	& \cmark &	& \cmark & \cmark &	&	&	& 											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-7	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-10	    		 & \xmark &	&	&	&	&	&	& \xmark &	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-16	    		 & \cmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-21	    		 &	&	&	&	& \cmark &	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-24	    		 &	&	&	& \xmark &	& \cmark & \cmark &	&	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-26	    		 &	& \cmark &	&	&	&	& \cmark &	&	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-27	    		 & \cmark &	&	&	&	&	&	&	&	&	& \xmark & 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-33	    		 & \cmark &	&	& \cmark & \cmark &	& \cmark &	&	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-35	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-38	    		 &	&	&	& (\cmark) &	&	& \cmark &	&	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-39	    		 & \cmark &	&	& \xmark &	& \xmark & \xmark &	&	&	&	& \xmark										& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-41	    		 & \cmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-43	    		 & \cmark & \cmark &	&	& \cmark &	& \cmark & \xmark &	&	&	& 										& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-44	    		 & \xmark &	&	&	&	&	& \xmark &	&	&	&	& \cmark												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-45	    		 & \xmark &	&	& (\cmark) &	&	&	&	&	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-46	    		 &	&	&	&	&	&	&	&	&	&	&	& \xmark														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-50	    		 & \cmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-51	    		 &	&	& \xmark & (\cmark) &	&	& \xmark & \cmark &	&	&	& \xmark									& \cmark &        \rmark &        \cmark &     \cmark &     \rmark &     \cmark &     \cmark &     \rmark &     \cmark &      \cmark &      \rmark &      \cmark &   \cmark &   \rmark &   \cmark &   \cmark &   \rmark &   \cmark &      \cmark &      \rmark &      \cmark \\
Lang-53	    		 &	&	&	&	&	&	&	&	&	&	&	& \xmark														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-55	    		 &	&	& \cmark & (\cmark) &	&	&	&	&	&	&	& \cmark											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-57	    		 &	& \cmark &	&	&	&	& \cmark & \xmark &	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-58	    		 & \cmark &	&	&	&	&	& \xmark &	&	&	&	& \cmark												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-59	    		 &	& \cmark & \cmark &	& \cmark &	& \cmark & \xmark &	&	&	& 											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-60	    		 & \cmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-61	    		 &	&	&	& \xmark &	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Lang-63	    		 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
\hline
Math-1	    		 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-2	    		 &	&	&	&	&	&	& \xmark &	& \xmark & \xmark & \xmark & 											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-3	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-4	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-5	    		 & \cmark & \cmark & \cmark & \cmark &	& \cmark & \cmark & \cmark & \cmark &	&	& 						& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-6	    		 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-8	    		 & \xmark &	&	&	&	&	&	&	& \xmark & \xmark &	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-20	    		 & \xmark &	&	&	&	&	& \xmark &	&	&	&	& 														& \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Math-22	    		 &	&	&	&	&	&	&	& \cmark &	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-25	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \rmark &        \rmark &        \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \rmark &      \rmark &      \rmark \\
Math-28	    		 & \xmark &	&	&	&	& \xmark &	&	& \xmark & \xmark & \xmark & 										& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-30	    		 &	& \cmark &	&	& \cmark &	& \cmark &	&	&	&	& 													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-32	    		 &	&	&	& (\cmark) &	&	& \xmark &	&	& \xmark &	& \xmark										& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-33	    		 & \cmark & \cmark & \cmark &	& \cmark &	& \cmark &	&	&	&	& \xmark								& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-34	    		 &	&	&	&	&	&	& \cmark & \xmark &	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-35	    		 & \cmark &	&	&	&	& \cmark &	&	&	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-40	    		 &	&	&	&	&	&	&	&	& \xmark & \xmark & \xmark & \xmark											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-41	    		 & \cmark &	&	&	& \cmark &	&	&	&	&	&	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-42	    		 &	&	&	&	&	&	&	&	&	&	&	& \xmark														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-49	    		 &	&	&	&	&	&	&	&	& \xmark & \xmark &	& \xmark												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-50	    		 & \cmark &	& \cmark & (\cmark) & \cmark &	& \cmark & \cmark & \cmark & \cmark & \xmark & \cmark			& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-53	    		 & \cmark & \cmark &	& (\cmark) & \cmark &	&	& \cmark & \cmark &	&	& 								& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-57	    		 & \cmark & \cmark &	&	& \cmark &	& \cmark &	&	&	& \xmark & \xmark								& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-58	    		 &	& \cmark &	&	&	&	& \cmark &	&	&	& \xmark & \xmark											& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-59	    		 & \cmark & \cmark & \cmark &	& \cmark &	& \cmark &	&	&	&	& 										& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-61	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-63	    		 & \cmark & \cmark &	&	&	&	& \xmark &	&	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-65	    		 &	& \cmark &	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-69	    		 &	&	&	&	&	&	&	&	&	&	&	& \xmark														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-70	    		  & \cmark & \cmark & \cmark &	& \cmark &	& \cmark & \xmark & \cmark &	&	& 							& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-71	    		 & \cmark &	&	&	&	&	&	&	& \xmark &	&	& \xmark												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-72	    		 & \xmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-73	    		 & \xmark &	& \xmark &	&	& \xmark & \xmark &	& \cmark &	&	& \xmark									& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-75	    		 & \cmark & \cmark &	&	&	&	& \cmark &	&	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-78	    		 &	&	&	&	&	&	&	&	& \xmark & \xmark &	& \xmark												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-79	    		 & \cmark & \xmark &	&	& \cmark &	&	&	&	&	&	& 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-80	    		 & \xmark & \xmark &	& (\cmark) & \cmark &	& \xmark &	& \xmark & \xmark &	& \xmark					& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-81	    		 & \xmark & \xmark &	&	&	& \xmark &	&	& \xmark & \xmark & \xmark & \xmark							& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-82	    		 & \xmark & \xmark & \cmark & (\cmark) &	& \cmark & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark	& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \rmark &   \rmark &      \cmark &      \cmark &      \cmark \\
Math-84	    		 &	&	&	&	&	&	&	&	& \xmark & \xmark & \xmark & 												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-85	    		 & \xmark & \cmark & \cmark & (\cmark) &	& \cmark & \cmark &	& \xmark & \xmark & \cmark & \xmark			& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-87	    		 &	&	&	&	&	&	&	&	&	&	&	& \xmark														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-88	    		 & \xmark &	&	&	&	&	&	&	&	&	& \xmark & \xmark												& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-89	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-90	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-93	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-95	    		 &	&	&	&	&	&	&	&	& \xmark & \xmark &	& 														& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-97	    		 &	&	&	&	&	& \xmark &	&	&	&	&	& \xmark													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-98	    		 & \cmark &	&	&	&	&	&	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-99	    		 &	&	&	&	&	& \cmark &	&	&	&	&	& 															& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Math-104			 &	&	&	&	&	&	& \xmark &	&	&	&	& \xmark													& \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Math-105			 &	&	&	& \xmark &	&	&	&	&	&	&	& \xmark													& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \rmark &   \rmark &      \cmark &      \cmark &      \cmark \\
\hline
Time-4	    		 &	&	& \xmark &	&	&	& \cmark &	& \xmark & \xmark &	& 				& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Time-7	    		 & \cmark &	&	&	&	&	&	&	&	&	&	& 							& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Time-11	    		 &	&	&	&	&	&	& \xmark &	& \xmark & \xmark & \xmark & \xmark		& \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
Time-15	    		 &	&	&	&	&	& \cmark & \cmark &	&	&	&	& 						& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
Time-19	    		 &	&	&	&	&	&	&	& \xmark &	&	&	& 							& \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\

\hline
\end{tabular}
	


==> table/aprPart2 <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c }
\hline
%\rotatebo\xmark[origin=l]{45}{Project}   &       \rotatebo\xmark[origin=l]{45}{SimFi\xmark}  &       \rotatebo\xmark[origin=l]{45}{CapGen}  &       \rotatebo\xmark[origin=l]{45}{SketchFi\xmark}       &       \rotatebo\xmark[origin=l]{45}{JAID}    &       \rotatebo\xmark[origin=l]{45}{ssFi\xmark}   &       \rotatebo\xmark[origin=l]{45}{ACS}     &       \rotatebo\xmark[origin=l]{45}{ELI\xmarkIR}  &       \rotatebo\xmark[origin=l]{45}{HDRepair}        &       \rotatebo\xmark[origin=l]{45}{\xmarkPAR}    &       \rotatebo\xmark[origin=l]{45}{jGenProg}        &       \rotatebo\xmark[origin=l]{45}{jKali}   &       \rotatebo\xmark[origin=l]{45}{jMutRepair}      &       \rotatebo\xmark[origin=l]{45}{Nopol}   &       \rotatebo\xmark[origin=l]{45}{MiningFi\xmarker} 
\rotatebox[origin=l]{0}{Project}	&	\rotatebox[origin=l]{90}{FixMiner}	&	\rotatebox[origin=l]{90}{SimFix}	&	\rotatebox[origin=l]{90}{CapGen}	&	\rotatebox[origin=l]{90}{SketchFix}	&	\rotatebox[origin=l]{90}{JAID}	&	\rotatebox[origin=l]{90}{ssFix}	&	\rotatebox[origin=l]{90}{ACS}	&	\rotatebox[origin=l]{90}{ELIXIR}	&	\rotatebox[origin=l]{90}{HDRepair}	&	\rotatebox[origin=l]{90}{jGenProg}	&	\rotatebox[origin=l]{90}{jKali}	&	\rotatebox[origin=l]{90}{jMutRepair}	&	\rotatebox[origin=l]{90}{Nopol}	\\
       
%\hline
\hline
\hline

Lang-60	&		&	\cmark	&		&		&		&		&		&		&		&		&		&		&		\\
Lang-61	&		&		&		&		&	\xmark	&		&		&		&		&		&		&		&		\\
Lang-63	&		&	\xmark	&		&		&		&		&		&		&		&		&		&		&		\\
\hline
Math-1	&		&	\xmark	&		&		&		&		&		&		&		&		&		&		&		\\
Math-2	&		&		&		&		&		&		&		&	\xmark	&		&	\xmark	&	\xmark	&	\xmark	&		\\
Math-3	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-4	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-5	&		&	\cmark	&	\cmark	&	\cmark	&	\cmark	&		&	\cmark	&	\cmark	&	\cmark	&	\cmark	&		&		&		\\
Math-6	&		&	\xmark	&		&		&		&		&		&		&		&		&		&		&		\\
Math-8	&		&	\xmark	&		&		&		&		&		&		&		&	\xmark	&	\xmark	&		&		\\
Math-10	&	\cmark	&		&		&		&		&		&		&		&		&		&		&		&		\\
Math-20	&		&	\xmark	&		&		&		&		&		&	\xmark	&		&		&		&		&		\\
Math-22	&	\cmark	&		&		&		&		&		&		&		&	\cmark	&		&		&		&		\\
Math-25	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-28	&		&	\xmark	&		&		&		&		&	\xmark	&		&		&	\xmark	&	\xmark	&	\xmark	&		\\
Math-30	&	\cmark	&		&	\cmark	&		&		&	\cmark	&		&	\cmark	&		&		&		&		&		\\
Math-32	&		&		&		&		&	(\cmark)	&		&		&	\xmark	&		&		&	\xmark	&		&	\xmark	\\
Math-33	&	\cmark	&	\cmark	&	\cmark	&	\cmark	&		&	\cmark	&		&	\cmark	&		&		&		&		&	\xmark	\\
Math-34	&	\cmark	&		&		&		&		&		&		&	\cmark	&	\xmark	&		&		&		&		\\
Math-35	&		&	\cmark	&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-40	&		&		&		&		&		&		&		&		&		&	\xmark	&	\xmark	&	\xmark	&	\xmark	\\
Math-41	&		&	\cmark	&		&		&		&	\cmark	&		&		&		&		&		&		&		\\
Math-42	&		&		&		&		&		&		&		&		&		&		&		&		&	\xmark	\\
Math-49	&		&		&		&		&		&		&		&		&		&	\xmark	&	\xmark	&		&	\xmark	\\
Math-50	&		&	\cmark	&		&	\cmark	&	(\cmark)	&	\cmark	&		&	\cmark	&	\cmark	&	\cmark	&	\cmark	&	\xmark	&	\cmark	\\
Math-53	&		&	\cmark	&	\cmark	&		&	(\cmark)	&	\cmark	&		&		&	\cmark	&	\cmark	&		&		&		\\
Math-57	&	\cmark	&	\cmark	&	\cmark	&		&		&	\cmark	&		&	\cmark	&		&		&		&	\xmark	&	\xmark	\\
Math-58	&	\cmark	&		&	\cmark	&		&		&		&		&	\cmark	&		&		&		&	\xmark	&	\xmark	\\
Math-59	&		&	\cmark	&	\cmark	&	\cmark	&		&	\cmark	&		&	\cmark	&		&		&		&		&		\\
Math-61	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-63	&		&	\cmark	&	\cmark	&		&		&		&		&	\xmark	&		&		&		&		&		\\
Math-65	&		&		&	\cmark	&		&		&		&		&		&		&		&		&		&		\\
Math-69	&		&		&		&		&		&		&		&		&		&		&		&		&	\xmark	\\
Math-70	&	\cmark	&	\cmark	&	\cmark	&	\cmark	&		&	\cmark	&		&	\cmark	&	\xmark	&	\cmark	&		&		&		\\
Math-71	&		&	\cmark	&		&		&		&		&		&		&		&	\xmark	&		&		&	\xmark	\\
Math-72	&		&	\xmark	&		&		&		&		&		&		&		&		&		&		&		\\
Math-73	&		&	\xmark	&		&	\xmark	&		&		&	\xmark	&	\xmark	&		&	\cmark	&		&		&	\xmark	\\
Math-75	&	\cmark	&	\cmark	&	\cmark	&		&		&		&		&	\cmark	&		&		&		&		&		\\
Math-78	&		&		&		&		&		&		&		&		&		&	\xmark	&	\xmark	&		&	\xmark	\\
Math-79	&	\cmark	&	\cmark	&	\xmark	&		&		&	\cmark	&		&		&		&		&		&		&		\\
Math-80	&		&	\xmark	&	\xmark	&		&	(\cmark)	&	\cmark	&		&	\xmark	&		&	\xmark	&	\xmark	&		&	\xmark	\\
Math-81	&	\xmark	&	\xmark	&	\xmark	&		&		&		&	\xmark	&		&		&	\xmark	&	\xmark	&	\xmark	&	\xmark	\\
Math-82	&	\cmark	&	\xmark	&	\xmark	&	\cmark	&	(\cmark)	&		&	\cmark	&	\cmark	&	\xmark	&	\xmark	&	\xmark	&	\cmark	&	\xmark	\\
Math-84	&	\xmark	&		&		&		&		&		&		&		&		&	\xmark	&	\xmark	&	\xmark	&		\\
Math-85	&	\cmark	&	\xmark	&	\cmark	&	\cmark	&	(\cmark)	&		&	\cmark	&	\cmark	&		&	\xmark	&	\xmark	&	\cmark	&	\xmark	\\
Math-87	&		&		&		&		&		&		&		&		&		&		&		&		&	\xmark	\\
Math-88	&		&	\xmark	&		&		&		&		&		&		&		&		&		&	\xmark	&	\xmark	\\
Math-89	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-90	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-93	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-95	&		&		&		&		&		&		&		&		&		&	\xmark	&	\xmark	&		&		\\
Math-97	&		&		&		&		&		&		&	\xmark	&		&		&		&		&		&	\xmark	\\
Math-98	&		&	\cmark	&		&		&		&		&		&		&		&		&		&		&		\\
Math-99	&		&		&		&		&		&		&	\cmark	&		&		&		&		&		&		\\
Math-104	&		&		&		&		&		&		&		&	\xmark	&		&		&		&		&	\xmark	\\
Math-105	&		&		&		&		&	\xmark	&		&		&		&		&		&		&		&	\xmark	\\
\hline
Time-4	&		&		&		&	\xmark	&		&		&		&	\cmark	&		&	\xmark	&	\xmark	&		&		\\
Time-7	&		&	\cmark	&		&		&		&		&		&		&		&		&		&		&		\\
Time-11	&		&		&		&		&		&		&		&	\xmark	&		&	\xmark	&	\xmark	&	\xmark	&	\xmark	\\
Time-15	&		&		&		&		&		&		&	\cmark	&	\cmark	&		&		&		&		&		\\
Time-19	&	\cmark	&		&		&		&		&		&		&		&	\xmark	&		&		&		&		\\
\hline
\end{tabular}

==> table/aprPartPosition <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c?c|c|c?c|c|c?c|c|c?c|c|c?c|c|c?c|c|c?c|c|c|}
\hline
&	&	&	&	&	&	&	&	&	&	&	&	&\multicolumn{3}{l?}{{GZ$^1$ Ochiai}} & \multicolumn{3}{l?}{{GZ$^2$ Ochiai}} \\
\hline
\rotatebox[origin=l]{0}{Project} & \rotatebox[origin=l]{90}{SimFix} & \rotatebox[origin=l]{90}{CapGen} & \rotatebox[origin=l]{90}{SketchFix} & \rotatebox[origin=l]{90}{JAID} & \rotatebox[origin=l]{90}{ssFix} & \rotatebox[origin=l]{90}{ACS} & \rotatebox[origin=l]{90}{ELIXIR} & \rotatebox[origin=l]{90}{HDRepair} & \rotatebox[origin=l]{90}{jGenProg} & \rotatebox[origin=l]{90}{jKali} & \rotatebox[origin=l]{90}{jMutRepair} & \rotatebox[origin=l]{90}{Nopol}	 & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Method}                   & \rotatebox[origin=l]{90}{Line}                    & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{Line}                \\
       
\hline
     Chart\_1 &      \cmark &      \cmark &         \cmark &  (\cmark) &     \cmark &     &      \cmark &        \rmark &        \rmark &     \rmark &          \cmark &       &        1 &        1 &       28 &       24 &       24 &       28 \\
     Chart\_3 &      \cmark &        &           &      &       &     &      \rmark &          &        \rmark &       &            &     \rmark &        1 &        1 &        7 &        1 &        1 &        4 \\
     Chart\_5 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &     \cmark &        1 &        1 &        7 &       12 &       66 &       72 \\
     Chart\_7 &      \cmark &        &           &      &       &     &        &          &        \rmark &       &          \rmark &       &        1 &        2 &       28 &        1 &        2 &       75 \\
     Chart\_8 &        &      \cmark &         \cmark &      &       &     &      \cmark &        \rmark &          &       &            &       &        0 &        0 &        0 &        1 &        1 &        1 \\
     Chart\_9 &        &        &         \cmark &  (\cmark) &       &     &      \cmark &          &          &       &            &       &        1 &        1 &        3 &        1 &        2 &       14 \\
    Chart\_11 &        &      \cmark &         \cmark &      &       &     &      \cmark &          &          &       &            &       &        1 &        1 &       15 &        1 &       24 &       28 \\
    Chart\_12 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        0 &        0 &      801 &     1092 &     1093 \\
    Chart\_13 &        &        &         \rmark &      &       &     &      \rmark &          &        \rmark &     \rmark &            &     \rmark &        1 &        1 &       17 &        5 &       35 &       51 \\
    Chart\_14 &      \rmark &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &        1 &       38 &      996 &      998 \\
    Chart\_15 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &       &        1 &       26 &       26 &     2143 &     8444 &     8445 \\
    Chart\_17 &        &        &           &      &       &     &      \rmark &          &          &       &            &       &        1 &        2 &        2 &       11 &       12 &       12 \\
    Chart\_18 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        1 &        6 &        1 &        1 &        3 \\
    Chart\_19 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &        5 &       37 &      833 &      833 \\
    Chart\_20 &      \cmark &        &         \cmark &      &     \cmark &     &        &          &          &       &            &       &        4 &        0 &        0 &       62 &       62 &       62 \\
    Chart\_21 &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        2 &        2 &        2 &        1 &       34 &       39 \\
    Chart\_22 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        1 &        1 &        1 &       53 &       58 \\
    Chart\_24 &        &      \cmark &         \cmark &    \cmark &     \cmark &     &        &          &          &       &            &       &        1 &        1 &        2 &        1 &        1 &        3 \\
    Chart\_25 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &          \rmark &     \rmark &        1 &       30 &       47 &     1325 &     3668 &     3913 \\
    Chart\_26 &        &        &         \rmark &    \cmark &       &     &        &          &          &     \rmark &          \rmark &     \rmark &      132 &      132 &      132 &        0 &        0 &        0 \\
   Closure\_5 &        &        &           &    \rmark &       &     &        &          &          &       &            &       &        8 &        0 &        0 &      561 &        0 &        0 \\
  Closure\_10 &        &        &           &      &       &     &        &        \rmark &          &       &            &       &        3 &       56 &      120 &        3 &       67 &      141 \\
  Closure\_14 &      \cmark &        &         \cmark &      &     \cmark &     &        &        \rmark &          &       &            &       &        1 &        2 &        3 &        2 &        3 &        3 \\
  Closure\_18 &        &        &           &    \cmark &       &     &        &          &          &       &            &       &       90 &     1495 &     1527 &       93 &     2320 &     2377 \\
  Closure\_31 &        &        &           &  (\cmark) &       &     &        &          &          &       &            &       &      215 &     1026 &     1043 &      214 &     1756 &     1802 \\
  Closure\_33 &        &        &           &    \cmark &       &     &        &          &          &       &            &       &        2 &        2 &      289 &        2 &        2 &      318 \\
  Closure\_40 &        &        &           &    \cmark &       &     &        &          &          &       &            &       &        9 &        0 &        0 &      104 &        0 &        0 \\
  Closure\_51 &        &        &           &      &       &     &        &        \rmark &          &       &            &       &       25 &       25 &       33 &       41 &       41 &       50 \\
  Closure\_57 &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        2 &        3 &        1 &        2 &        7 \\
  Closure\_62 &      \cmark &        &         \cmark &  (\cmark) &       &     &        &        \rmark &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        4 \\
  Closure\_63 &      \cmark &        &           &  (\cmark) &       &     &        &          &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        4 \\
  Closure\_70 &        &        &         \rmark &    \cmark &       &     &        &        \rmark &          &       &            &       &      143 &        0 &        0 &      264 &        0 &        0 \\
  Closure\_73 &      \cmark &        &         \rmark &    \cmark &       &     &        &        \rmark &          &       &            &       &        1 &        7 &       10 &        1 &        1 &       16 \\
  Closure\_79 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        0 &        0 &        0 &        1 &       37 &       37 \\
 Closure\_106 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        0 &        0 &        0 &        3 &        4 &        4 \\
 Closure\_115 &      \cmark &        &           &      &     \cmark &     &        &          &          &       &            &       &        1 &        1 &        1 &        8 &        8 &        8 \\
 Closure\_125 &        &        &           &    \rmark &       &     &        &          &          &       &            &       &        4 &      142 &      145 &        5 &      166 &      170 \\
 Closure\_126 &        &        &         \cmark &  (\cmark) &       &     &        &        \rmark &          &       &            &       &        1 &        1 &        1 &        6 &        6 &        6 \\
      Lang\_6 &        &      \cmark &         \cmark &      &     \cmark &     &      \cmark &        \cmark &          &       &            &       &        0 &        0 &        0 &       54 &       73 &       74 \\
      Lang\_7 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &      373 &        0 &        0 &        1 &        1 &       25 \\
     Lang\_10 &      \rmark &        &           &      &       &     &        &        \rmark &          &       &            &       &      114 &        0 &        0 &        1 &       64 &       64 \\
     Lang\_16 &      \cmark &        &           &      &       &     &        &          &          &       &            &       &      322 &        0 &        0 &        1 &        1 &       27 \\
     Lang\_21 &        &        &           &      &     \cmark &     &        &          &          &       &            &       &        1 &        0 &        0 &        1 &        1 &        2 \\
     Lang\_24 &        &        &           &    \rmark &       &   \cmark &      \cmark &          &          &       &            &       &      259 &      618 &        0 &        1 &       14 &       64 \\
     Lang\_26 &        &      \cmark &           &      &       &     &      \cmark &          &          &       &            &       &       21 &        0 &        0 &        1 &      112 &      112 \\
     Lang\_27 &      \cmark &        &           &      &       &     &        &          &          &       &          \rmark &       &      262 &      269 &        0 &        1 &        1 &       56 \\
     Lang\_33 &      \cmark &        &           &    \cmark &     \cmark &     &      \cmark &          &          &       &            &       &       14 &        0 &        0 &        1 &        1 &        7 \\
     Lang\_35 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &       53 &        0 &        0 &        1 &        1 &        2 \\
     Lang\_38 &        &        &           &  (\cmark) &       &     &      \cmark &          &          &       &            &       &      104 &        0 &        0 &        1 &        3 &        3 \\
     Lang\_39 &      \cmark &        &           &    \rmark &       &   \rmark &      \rmark &          &          &       &            &     \rmark &      203 &        0 &        0 &        1 &        2 &       27 \\
     Lang\_41 &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        5 &        7 &        1 &        5 &        6 \\
     Lang\_43 &      \cmark &      \cmark &           &      &     \cmark &     &      \cmark &        \rmark &          &       &            &       &        1 &        1 &        1 &        1 &       26 &       29 \\
     Lang\_44 &      \rmark &        &           &      &       &     &      \rmark &          &          &       &            &     \cmark &        1 &        5 &       20 &        1 &        1 &        3 \\
     Lang\_45 &      \rmark &        &           &  (\cmark) &       &     &        &          &          &       &            &       &        1 &        1 &       16 &        1 &        1 &        5 \\
     Lang\_46 &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        1 &        1 &        3 &        1 &        1 &        1 \\
     Lang\_50 &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        9 &       15 &        1 &        8 &        8 \\
     Lang\_51 &        &        &         \rmark &  (\cmark) &       &     &      \rmark &        \cmark &          &       &            &     \rmark &        1 &        1 &        0 &        1 &        1 &        0 \\
     Lang\_53 &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        1 &        1 &       32 &        1 &        1 &       16 \\
     Lang\_55 &        &        &         \cmark &  (\cmark) &       &     &        &          &          &       &            &     \cmark &        1 &        7 &        9 &        1 &        6 &        7 \\
     Lang\_57 &        &      \cmark &           &      &       &     &      \cmark &        \rmark &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        1 \\
     Lang\_58 &      \cmark &        &           &      &       &     &      \rmark &          &          &       &            &     \cmark &        1 &        2 &        8 &        1 &        1 &       20 \\
     Lang\_59 &        &      \cmark &         \cmark &      &     \cmark &     &      \cmark &        \rmark &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        6 \\
     Lang\_60 &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        1 &        3 &        1 &        1 &        2 \\
     Lang\_61 &        &        &           &    \rmark &       &     &        &          &          &       &            &       &        1 &       14 &       19 &        1 &       14 &       21 \\
     Lang\_63 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        1 \\
      Math\_1 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &       20 &        0 &        0 &       12 &       14 &       14 \\
      Math\_2 &        &        &           &      &       &     &      \rmark &          &        \rmark &     \rmark &          \rmark &       &        1 &       11 &       11 &       44 &       44 &       44 \\
      Math\_3 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &       16 &        1 &        1 &        3 \\
      Math\_4 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &        1 &        1 &        3 &        6 \\
      Math\_5 &      \cmark &      \cmark &         \cmark &    \cmark &       &   \cmark &      \cmark &        \cmark &        \cmark &       &            &       &        1 &        2 &        2 &        1 &        1 &        1 \\
      Math\_6 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        2 &      205 &        1 &        2 &      177 \\
      Math\_8 &      \rmark &        &           &      &       &     &        &          &        \rmark &     \rmark &            &       &        1 &        1 &        3 &        1 &        3 &        4 \\
     Math\_20 &      \rmark &        &           &      &       &     &      \rmark &          &          &       &            &       &        1 &        0 &        0 &        1 &        0 &        0 \\
     Math\_22 &        &        &           &      &       &     &        &        \cmark &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_25 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        0 &        0 &        0 &        0 &        0 &        0 \\
     Math\_28 &      \rmark &        &           &      &       &   \rmark &        &          &        \rmark &     \rmark &          \rmark &       &        6 &        6 &        6 &       13 &       13 &       13 \\
     Math\_30 &        &      \cmark &           &      &     \cmark &     &      \cmark &          &          &       &            &       &        1 &        4 &        9 &      142 &      161 &      161 \\
     Math\_32 &        &        &           &  (\cmark) &       &     &      \rmark &          &          &     \rmark &            &     \rmark &        1 &        3 &        3 &        5 &        5 &        6 \\
     Math\_33 &      \cmark &      \cmark &         \cmark &      &     \cmark &     &      \cmark &          &          &       &            &     \rmark &        2 &        4 &       31 &        2 &        6 &       44 \\
     Math\_34 &        &        &           &      &       &     &      \cmark &        \rmark &          &       &            &       &        1 &        1 &        1 &        1 &        3 &        3 \\
     Math\_35 &      \cmark &        &           &      &       &   \cmark &        &          &          &       &            &       &        0 &        0 &        0 &        1 &        3 &        5 \\
     Math\_40 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &          \rmark &     \rmark &        1 &       23 &       24 &       24 &       33 &       34 \\
     Math\_41 &      \cmark &        &           &      &     \cmark &     &        &          &          &       &            &       &        1 &        2 &        6 &        1 &       37 &       49 \\
     Math\_42 &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        1 &       23 &       26 &        3 &       57 &       66 \\
     Math\_49 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &     \rmark &        3 &        4 &        7 &        5 &        5 &        7 \\
     Math\_50 &      \cmark &        &         \cmark &  (\cmark) &     \cmark &     &      \cmark &        \cmark &        \cmark &     \cmark &          \rmark &     \cmark &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_53 &      \cmark &      \cmark &           &  (\cmark) &     \cmark &     &        &        \cmark &        \cmark &       &            &       &        1 &        1 &        1 &        1 &        1 &        2 \\
     Math\_57 &      \cmark &      \cmark &           &      &     \cmark &     &      \cmark &          &          &       &          \rmark &     \rmark &        1 &        1 &       14 &        1 &        4 &        4 \\
     Math\_58 &        &      \cmark &           &      &       &     &      \cmark &          &          &       &          \rmark &     \rmark &        6 &        6 &        6 &      223 &      223 &      223 \\
     Math\_59 &      \cmark &      \cmark &         \cmark &      &     \cmark &     &      \cmark &          &          &       &            &       &        1 &        1 &        1 &        1 &        2 &        2 \\
     Math\_61 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        0 &        0 &        0 &        1 &        1 &        1 \\
     Math\_63 &      \cmark &      \cmark &           &      &       &     &      \rmark &          &          &       &            &       &        1 &        8 &        8 &        1 &        1 &        1 \\
     Math\_65 &        &      \cmark &           &      &       &     &        &          &          &       &            &       &        1 &        8 &        9 &       12 &       12 &       15 \\
     Math\_69 &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        1 &        1 &        2 &        1 &       48 &       57 \\
     Math\_70 &      \cmark &      \cmark &         \cmark &      &     \cmark &     &      \cmark &        \rmark &        \cmark &       &            &       &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_71 &      \cmark &        &           &      &       &     &        &          &        \rmark &       &            &     \rmark &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_72 &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        3 &        4 &        1 &        1 &        1 \\
     Math\_73 &      \rmark &        &         \rmark &      &       &   \rmark &      \rmark &          &        \cmark &       &            &     \rmark &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_75 &      \cmark &      \cmark &           &      &       &     &      \cmark &          &          &       &            &       &        1 &        2 &        2 &        1 &        1 &        1 \\
     Math\_78 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &     \rmark &       17 &       21 &       32 &       67 &       67 &      109 \\
     Math\_79 &      \cmark &      \rmark &           &      &     \cmark &     &        &          &          &       &            &       &       23 &       23 &       25 &       29 &       29 &       29 \\
     Math\_80 &      \rmark &      \rmark &           &  (\cmark) &     \cmark &     &      \rmark &          &        \rmark &     \rmark &            &     \rmark &        1 &       11 &       18 &        1 &       14 &       14 \\
     Math\_81 &      \rmark &      \rmark &           &      &       &   \rmark &        &          &        \rmark &     \rmark &          \rmark &     \rmark &        1 &        1 &        6 &        1 &        1 &       10 \\
     Math\_82 &      \rmark &      \rmark &         \cmark &  (\cmark) &       &   \cmark &      \cmark &        \rmark &        \rmark &     \rmark &          \cmark &     \rmark &        2 &       53 &       60 &        1 &       76 &       84 \\
     Math\_84 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &          \rmark &       &        1 &       13 &       30 &        5 &       18 &      134 \\
     Math\_85 &      \rmark &      \cmark &         \cmark &  (\cmark) &       &   \cmark &      \cmark &          &        \rmark &     \rmark &          \cmark &     \rmark &        1 &        1 &       36 &       11 &       11 &       90 \\
     Math\_87 &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        1 &       99 &      100 &        2 &      109 &      111 \\
     Math\_88 &      \rmark &        &           &      &       &     &        &          &          &       &          \rmark &     \rmark &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_89 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_90 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &        4 &        1 &        1 &        3 \\
     Math\_93 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &        2 &        1 &        1 &        2 \\
     Math\_95 &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &       &        2 &        2 &        3 &        8 &       11 &       12 \\
     Math\_97 &        &        &           &      &       &   \rmark &        &          &          &       &            &     \rmark &        1 &        1 &        1 &        1 &        1 &        1 \\
     Math\_98 &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        1 &        6 &        1 &        1 &        4 \\
     Math\_99 &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 &        1 &        1 &        1 &        4 \\
    Math\_104 &        &        &           &      &       &     &      \rmark &          &          &       &            &     \rmark &        1 &        0 &        0 &        1 &        0 &        0 \\
    Math\_105 &        &        &           &    \rmark &       &     &        &          &          &       &            &     \rmark &        1 &        1 &        1 &        1 &       25 &       25 \\
      Time\_4 &        &        &         \rmark &      &       &     &      \cmark &          &        \rmark &     \rmark &            &       &       36 &       36 &      208 &        6 &        6 &       31 \\
      Time\_7 &      \cmark &        &           &      &       &     &        &          &          &       &            &       &       48 &       48 &       51 &       10 &       10 &       14 \\
     Time\_11 &        &        &           &      &       &     &      \rmark &          &        \rmark &     \rmark &          \rmark &     \rmark &        4 &        0 &        0 &       51 &        0 &        0 \\
     Time\_15 &        &        &           &      &       &   \cmark &      \cmark &          &          &       &            &       &        1 &        1 &      115 &        1 &        1 &        2 \\
     Time\_19 &        &        &           &      &       &     &        &        \rmark &          &       &            &       &        5 &      449 &      449 &      104 &      620 &      620 \\


\hline
\end{tabular}
	


==> table/flPart1 <==
\begin{tabular}{|l|l|l?l|l|l ?l|l|l?l|l|l?l|l|l?l|l|l?l|l|l|}
\hline
\multicolumn{3}{l?}{{Tarantula}} & \multicolumn{3}{l?}{{Ochiai}} & \multicolumn{3}{l?}{{Dstar2}} & \multicolumn{3}{l?}{{Barinel}} & \multicolumn{3}{l?}{{Opt2}} & \multicolumn{3}{l?}{{Muse}} & \multicolumn{3}{l}{{Jaccard}} \\ 
\hline

 \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                    & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                  & \rotatebox[origin=l]{90}{Line}                 & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                   & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                 & \rotatebox[origin=l]{90}{File}                    & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                   \\ 
 \hline
 \hline
          \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \rmark &     \rmark &      \cmark &      \cmark &      \cmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \rmark &     \rmark &      \cmark &      \cmark &      \cmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
         \rmark &        \rmark &        \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &      \rmark &      \rmark &      \rmark &   \rmark &   \rmark &   \rmark &   \rmark &   \rmark &   \rmark &      \rmark &      \rmark &      \rmark \\
 \hline
         \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
\hline
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \rmark &        \cmark &     \cmark &     \rmark &     \cmark &     \cmark &     \rmark &     \cmark &      \cmark &      \rmark &      \cmark &   \cmark &   \rmark &   \cmark &   \cmark &   \rmark &   \cmark &      \cmark &      \rmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
         \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
\hline
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \rmark &        \rmark &        \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \rmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \rmark &   \rmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \rmark &   \rmark &      \cmark &      \cmark &      \cmark \\
 \hline
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\

\hline
                             
\end{tabular}


==> table/flPart2 <==
\begin{tabular}{l|l|l?l|l|l ?l|l|l?l|l|l?l|l|l?l|l|l?l|l|l}
\toprule
\multicolumn{3}{l?}{{Tarantula}} & \multicolumn{3}{l?}{{Ochiai}} & \multicolumn{3}{l?}{{Dstar2}} & \multicolumn{3}{l?}{{Barinel}} & \multicolumn{3}{l?}{{Opt2}} & \multicolumn{3}{l?}{{Muse}} & \multicolumn{3}{l?}{{Jaccard}} \\ 
 \hline

 \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                    & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                  & \rotatebox[origin=l]{90}{Line}                 & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                   & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                  & \rotatebox[origin=l]{90}{File}                   & \rotatebox[origin=l]{90}{Line}                  & \rotatebox[origin=l]{90}{Method}                 & \rotatebox[origin=l]{90}{File}                    & \rotatebox[origin=l]{90}{Line}                   & \rotatebox[origin=l]{90}{Method}                   \\ 
 \hline
          \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
    \hline
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \rmark &        \rmark &        \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \rmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \rmark &   \rmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\

        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \rmark &   \rmark &      \cmark &      \cmark &      \cmark \\
\hline

       \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
      \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
      \cmark &        \rmark &        \rmark &     \cmark &     \rmark &     \rmark &     \cmark &     \rmark &     \rmark &      \cmark &      \rmark &      \rmark &   \cmark &   \rmark &   \rmark &   \cmark &   \rmark &   \rmark &      \cmark &      \rmark &      \rmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
        \cmark &        \cmark &        \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &     \cmark &      \cmark &      \cmark &      \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &   \cmark &      \cmark &      \cmark &      \cmark \\
                       
\end{tabular}


==> table/localizable <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|r|r|}
\toprule
        \rotatebox[origin=l]{0}{Bug ID} & \rotatebox[origin=l]{90}{FixMiner} & \rotatebox[origin=l]{90}{LSRepair} & \rotatebox[origin=l]{90}{SimFix} & \rotatebox[origin=l]{90}{CapGen} & \rotatebox[origin=l]{90}{SketchFix} & \rotatebox[origin=l]{90}{JAID} & \rotatebox[origin=l]{90}{ssFix} & \rotatebox[origin=l]{90}{ACS} & \rotatebox[origin=l]{90}{ELIXIR} & \rotatebox[origin=l]{90}{HDRepair} & \rotatebox[origin=l]{90}{jGenProg} & \rotatebox[origin=l]{90}{jKali} & \rotatebox[origin=l]{90}{jMutRepair} & \rotatebox[origin=l]{90}{Nopol} &  \rotatebox[origin=l]{90}{GZ$^1$ \& Ochiai} &  \rotatebox[origin=l]{90}{GZ$^2$ \& Ochiai} \\
\midrule
     Chart-1 &        \cmark &        \cmark &      \cmark &      \cmark &         \cmark &  (\cmark) &     \cmark &     &      \cmark &        \rmark &        \rmark &     \rmark &          \cmark &       &       28 &       28 \\
     Chart-3 &          &          &      \cmark &        &           &      &       &     &      \rmark &          &        \rmark &       &            &     \rmark &        7 &        4 \\
     Chart-4 &        \cmark &        \cmark &        &        &           &      &       &     &        &          &          &       &            &       &       49 &      173 \\
     Chart-5 &          &          &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &     \cmark &        7 &       72 \\
     Chart-6 &          &        \rmark &        &        &           &      &       &     &        &          &          &       &            &       &       49 &      224 \\
     Chart-7 &          &          &      \cmark &        &           &      &       &     &        &          &        \rmark &       &          \rmark &       &       28 &       75 \\
     Chart-9 &          &          &        &        &         \cmark &  (\cmark) &       &     &      \cmark &          &          &       &            &       &        3 &       14 \\
    Chart-10 &          &        \rmark &        &        &           &      &       &     &        &          &          &       &            &       &        1 &        3 \\
    Chart-11 &        \cmark &        \cmark &        &      \cmark &         \cmark &      &       &     &      \cmark &          &          &       &            &       &       15 &       28 \\
    Chart-13 &        \rmark &          &        &        &         \rmark &      &       &     &      \rmark &          &        \rmark &     \rmark &            &     \rmark &       17 &       51 \\
    Chart-14 &          &          &      \rmark &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &      998 \\
    Chart-15 &          &          &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &       &       26 &     8445 \\
    Chart-17 &          &        \rmark &        &        &           &      &       &     &      \rmark &          &          &       &            &       &        2 &       12 \\
    Chart-18 &          &        \rmark &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        6 &        3 \\
    Chart-19 &          &          &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        5 &      833 \\
    Chart-21 &          &          &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        2 &       39 \\
    Chart-22 &          &          &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &       58 \\
    Chart-24 &        \cmark &          &        &      \cmark &         \cmark &    \cmark &     \cmark &     &        &          &          &       &            &       &        2 &        3 \\
    Chart-25 &        \rmark &          &        &        &           &      &       &     &        &          &        \rmark &     \rmark &          \rmark &     \rmark &       47 &     3913 \\
    Chart-26 &        \cmark &        \rmark &        &        &         \rmark &    \cmark &       &     &        &          &          &     \rmark &          \rmark &     \rmark &      132 &        0 \\
  Closure-10 &        \cmark &          &        &        &           &      &       &     &        &        \rmark &          &       &            &       &      120 &      141 \\
  Closure-14 &          &          &      \cmark &        &         \cmark &      &     \cmark &     &        &        \rmark &          &       &            &       &        3 &        3 \\
  Closure-18 &          &          &        &        &           &    \cmark &       &     &        &          &          &       &            &       &     1527 &     2377 \\
  Closure-31 &          &          &        &        &           &  (\cmark) &       &     &        &          &          &       &            &       &     1043 &     1802 \\
  Closure-33 &          &          &        &        &           &    \cmark &       &     &        &          &          &       &            &       &      289 &      318 \\
  Closure-38 &        \cmark &          &        &        &           &      &       &     &        &          &          &       &            &       &       34 &       49 \\
  Closure-51 &          &          &        &        &           &      &       &     &        &        \rmark &          &       &            &       &       33 &       50 \\
  Closure-57 &          &          &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        3 &        7 \\
  Closure-62 &        \cmark &          &      \cmark &        &         \cmark &  (\cmark) &       &     &        &        \rmark &          &       &            &       &        1 &        4 \\
  Closure-63 &        \cmark &          &      \cmark &        &           &  (\cmark) &       &     &        &          &          &       &            &       &        1 &        4 \\
  Closure-73 &        \cmark &          &      \cmark &        &         \rmark &    \cmark &       &     &        &        \rmark &          &       &            &       &       10 &       16 \\
 Closure-115 &          &          &      \cmark &        &           &      &     \cmark &     &        &          &          &       &            &       &        1 &        8 \\
 Closure-125 &          &          &        &        &           &    \rmark &       &     &        &          &          &       &            &       &      145 &      170 \\
 Closure-126 &          &          &        &        &         \cmark &  (\cmark) &       &     &        &        \rmark &          &       &            &       &        1 &        6 \\
      Lang-2 &          &        \rmark &        &        &           &      &       &     &        &          &          &       &            &       &      128 &       17 \\
     Lang-40 &          &        \rmark &        &        &           &      &       &     &        &          &          &       &            &       &        1 &        2 \\
     Lang-41 &          &        \rmark &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        7 &        6 \\
     Lang-43 &        \rmark &          &      \cmark &      \cmark &           &      &     \cmark &     &      \cmark &        \rmark &          &       &            &       &        1 &       29 \\
     Lang-44 &          &          &      \rmark &        &           &      &       &     &      \rmark &          &          &       &            &     \cmark &       20 &        3 \\
     Lang-45 &          &          &      \rmark &        &           &  (\cmark) &       &     &        &          &          &       &            &       &       16 &        5 \\
     Lang-46 &          &        \cmark &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        3 &        1 \\
     Lang-48 &          &        \cmark &        &        &           &      &       &     &        &          &          &       &            &       &        2 &        2 \\
     Lang-50 &          &          &      \cmark &        &           &      &       &     &        &          &          &       &            &       &       15 &        8 \\
     Lang-52 &          &        \cmark &        &        &           &      &       &     &        &          &          &       &            &       &       13 &       25 \\
     Lang-53 &          &          &        &        &           &      &       &     &        &          &          &       &            &     \rmark &       32 &       16 \\
     Lang-54 &          &        \cmark &        &        &           &      &       &     &        &          &          &       &            &       &        2 &        4 \\
     Lang-55 &          &        \rmark &        &        &         \cmark &  (\cmark) &       &     &        &          &          &       &            &     \cmark &        9 &        7 \\
     Lang-57 &        \cmark &          &        &      \cmark &           &      &       &     &      \cmark &        \rmark &          &       &            &       &        1 &        1 \\
     Lang-58 &          &          &      \cmark &        &           &      &       &     &      \rmark &          &          &       &            &     \cmark &        8 &       20 \\
     Lang-59 &        \cmark &          &        &      \cmark &         \cmark &      &     \cmark &     &      \cmark &        \rmark &          &       &            &       &        1 &        6 \\
     Lang-60 &          &        \rmark &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        3 &        2 \\
     Lang-61 &          &          &        &        &           &    \rmark &       &     &        &          &          &       &            &       &       19 &       21 \\
     Lang-62 &          &        \rmark &        &        &           &      &       &     &        &          &          &       &            &       &        7 &        7 \\
     Lang-63 &          &          &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        1 &        1 \\
      Math-2 &          &          &        &        &           &      &       &     &      \rmark &          &        \rmark &     \rmark &          \rmark &       &       11 &       44 \\
      Math-3 &          &          &        &        &           &      &       &   \cmark &        &          &          &       &            &       &       16 &        3 \\
      Math-4 &          &          &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        6 \\
      Math-5 &          &          &      \cmark &      \cmark &         \cmark &    \cmark &       &   \cmark &      \cmark &        \cmark &        \cmark &       &            &       &        2 &        1 \\
      Math-6 &          &          &      \rmark &        &           &      &       &     &        &          &          &       &            &       &      205 &      177 \\
      Math-8 &          &          &      \rmark &        &           &      &       &     &        &          &        \rmark &     \rmark &            &       &        3 &        4 \\
     Math-10 &        \cmark &          &        &        &           &      &       &     &        &          &          &       &            &       &        1 &       17 \\
     Math-11 &          &        \rmark &        &        &           &      &       &     &        &          &          &       &            &       &        9 &       29 \\
     Math-16 &          &        \rmark &        &        &           &      &       &     &        &          &          &       &            &       &        5 &        5 \\
     Math-22 &        \cmark &          &        &        &           &      &       &     &        &        \cmark &          &       &            &       &        1 &        1 \\
     Math-28 &          &        \rmark &      \rmark &        &           &      &       &   \rmark &        &          &        \rmark &     \rmark &          \rmark &       &        6 &       13 \\
     Math-30 &        \cmark &          &        &      \cmark &           &      &     \cmark &     &      \cmark &          &          &       &            &       &        9 &      161 \\
     Math-32 &          &          &        &        &           &  (\cmark) &       &     &      \rmark &          &          &     \rmark &            &     \rmark &        3 &        6 \\
     Math-33 &        \cmark &          &      \cmark &      \cmark &         \cmark &      &     \cmark &     &      \cmark &          &          &       &            &     \rmark &       31 &       44 \\
     Math-34 &        \cmark &          &        &        &           &      &       &     &      \cmark &        \rmark &          &       &            &       &        1 &        3 \\
     Math-40 &          &          &        &        &           &      &       &     &        &          &        \rmark &     \rmark &          \rmark &     \rmark &       24 &       34 \\
     Math-41 &          &          &      \cmark &        &           &      &     \cmark &     &        &          &          &       &            &       &        6 &       49 \\
     Math-42 &          &          &        &        &           &      &       &     &        &          &          &       &            &     \rmark &       26 &       66 \\
     Math-49 &          &          &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &     \rmark &        7 &        7 \\
     Math-50 &          &          &      \cmark &        &         \cmark &  (\cmark) &     \cmark &     &      \cmark &        \cmark &        \cmark &     \cmark &          \rmark &     \cmark &        1 &        1 \\
     Math-53 &          &          &      \cmark &      \cmark &           &  (\cmark) &     \cmark &     &        &        \cmark &        \cmark &       &            &       &        1 &        2 \\
     Math-57 &        \cmark &          &      \cmark &      \cmark &           &      &     \cmark &     &      \cmark &          &          &       &          \rmark &     \rmark &       14 &        4 \\
     Math-58 &        \cmark &          &        &      \cmark &           &      &       &     &      \cmark &          &          &       &          \rmark &     \rmark &        6 &      223 \\
     Math-59 &          &          &      \cmark &      \cmark &         \cmark &      &     \cmark &     &      \cmark &          &          &       &            &       &        1 &        2 \\
     Math-63 &          &        \cmark &      \cmark &      \cmark &           &      &       &     &      \rmark &          &          &       &            &       &        8 &        1 \\
     Math-65 &          &          &        &      \cmark &           &      &       &     &        &          &          &       &            &       &        9 &       15 \\
     Math-69 &          &          &        &        &           &      &       &     &        &          &          &       &            &     \rmark &        2 &       57 \\
     Math-70 &        \cmark &        \cmark &      \cmark &      \cmark &         \cmark &      &     \cmark &     &      \cmark &        \rmark &        \cmark &       &            &       &        1 &        1 \\
     Math-71 &          &          &      \cmark &        &           &      &       &     &        &          &        \rmark &       &            &     \rmark &        1 &        1 \\
     Math-72 &          &          &      \rmark &        &           &      &       &     &        &          &          &       &            &       &        4 &        1 \\
     Math-73 &          &          &      \rmark &        &         \rmark &      &       &   \rmark &      \rmark &          &        \cmark &       &            &     \rmark &        1 &        1 \\
     Math-75 &        \cmark &        \cmark &      \cmark &      \cmark &           &      &       &     &      \cmark &          &          &       &            &       &        2 &        1 \\
     Math-78 &          &          &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &     \rmark &       32 &      109 \\
     Math-79 &        \cmark &        \cmark &      \cmark &      \rmark &           &      &     \cmark &     &        &          &          &       &            &       &       25 &       29 \\
     Math-80 &          &        \rmark &      \rmark &      \rmark &           &  (\cmark) &     \cmark &     &      \rmark &          &        \rmark &     \rmark &            &     \rmark &       18 &       14 \\
     Math-81 &        \rmark &          &      \rmark &      \rmark &           &      &       &   \rmark &        &          &        \rmark &     \rmark &          \rmark &     \rmark &        6 &       10 \\
     Math-82 &        \cmark &          &      \rmark &      \rmark &         \cmark &  (\cmark) &       &   \cmark &      \cmark &        \rmark &        \rmark &     \rmark &          \cmark &     \rmark &       60 &       84 \\
     Math-84 &        \rmark &          &        &        &           &      &       &     &        &          &        \rmark &     \rmark &          \rmark &       &       30 &      134 \\
     Math-85 &        \cmark &          &      \rmark &      \cmark &         \cmark &  (\cmark) &       &   \cmark &      \cmark &          &        \rmark &     \rmark &          \cmark &     \rmark &       36 &       90 \\
     Math-87 &          &          &        &        &           &      &       &     &        &          &          &       &            &     \rmark &      100 &      111 \\
     Math-88 &          &          &      \rmark &        &           &      &       &     &        &          &          &       &          \rmark &     \rmark &        1 &        1 \\
     Math-89 &          &        \cmark &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        1 \\
     Math-90 &          &          &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        4 &        3 \\
     Math-91 &          &        \cmark &        &        &           &      &       &     &        &          &          &       &            &       &        2 &        1 \\
     Math-93 &          &        \rmark &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        2 &        2 \\
     Math-94 &          &        \cmark &        &        &           &      &       &     &        &          &          &       &            &       &       21 &       21 \\
     Math-95 &          &        \rmark &        &        &           &      &       &     &        &          &        \rmark &     \rmark &            &       &        3 &       12 \\
     Math-97 &          &          &        &        &           &      &       &   \rmark &        &          &          &       &            &     \rmark &        1 &        1 \\
     Math-98 &          &          &      \cmark &        &           &      &       &     &        &          &          &       &            &       &        6 &        4 \\
     Math-99 &          &        \rmark &        &        &           &      &       &   \cmark &        &          &          &       &            &       &        1 &        4 \\
    Math-105 &          &          &        &        &           &    \rmark &       &     &        &          &          &       &            &     \rmark &        1 &       25 \\
  Mockito-13 &          &        \cmark &        &        &           &      &       &     &        &          &          &       &            &       &       70 &      135 \\
      Time-4 &          &          &        &        &         \rmark &      &       &     &      \cmark &          &        \rmark &     \rmark &            &       &      208 &       31 \\
      Time-7 &          &          &      \cmark &        &           &      &       &     &        &          &          &       &            &       &       51 &       14 \\
     Time-15 &          &          &        &        &           &      &       &   \cmark &      \cmark &          &          &       &            &       &      115 &        2 \\
     Time-19 &        \cmark &          &        &        &           &      &       &     &        &        \rmark &          &       &            &       &      449 &      620 \\
\bottomrule
\end{tabular}


==> table/nonlocalizable <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|r|r|}
\hline
        \rotatebox[origin=l]{0}{Bug ID} & \rotatebox[origin=l]{90}{FixMiner} & \rotatebox[origin=l]{90}{LSRepair} & \rotatebox[origin=l]{90}{SimFix} & \rotatebox[origin=l]{90}{CapGen} & \rotatebox[origin=l]{90}{SketchFix} & \rotatebox[origin=l]{90}{JAID} & \rotatebox[origin=l]{90}{ssFix} & \rotatebox[origin=l]{90}{ACS} & \rotatebox[origin=l]{90}{ELIXIR} & \rotatebox[origin=l]{90}{HDRepair} & \rotatebox[origin=l]{90}{jGenProg} & \rotatebox[origin=l]{90}{jKali} & \rotatebox[origin=l]{90}{jMutRepair} & \rotatebox[origin=l]{90}{Nopol} &  \rotatebox[origin=l]{90}{GZ$^1$ \& Ochiai} &  \rotatebox[origin=l]{90}{GZ$^2$ \& Ochiai} \\
\hline
     Chart-8 &          &          &        &      \ding{108} &         \ding{108} &      &       &     &      \ding{108} &        \ding{109} &          &       &            &       &       {\bf \color{red}0}&        1 \\
    Chart-12 &        \ding{109} &          &      \ding{109} &        &           &      &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&     1093 \\
    Chart-20 &          &          &      \ding{108} &        &         \ding{108} &      &     \ding{108} &     &        &          &          &       &            &       &       {\bf \color{red}0}&       62 \\
\hline
   Closure-5 &          &          &        &        &           &    \ding{109} &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
   Closure-7 &          &          &        &        &           &      &     \ding{109} &     &        &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
  Closure-40 &          &          &        &        &           &    \ding{108} &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
  Closure-42 &          &          &        &        &           &      &     \ding{109} &     &        &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
  Closure-70 &          &          &        &        &         \ding{109} &    \ding{108} &       &     &        &        \ding{109} &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
  Closure-79 &          &          &      \ding{109} &        &           &      &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&       37 \\
 Closure-106 &          &          &      \ding{109} &        &           &      &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&        4 \\
 Closure-111 &          &          &        &        &           &      &     \ding{109} &     &        &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
\hline
      Lang-6 &          &          &        &      \ding{108} &         \ding{108} &      &     \ding{108} &     &      \ding{108} &        \ding{108} &          &       &            &       &       {\bf \color{red}0}&       74 \\
      Lang-7 &          &          &        &        &           &      &       &   \ding{108} &        &          &          &       &            &       &       {\bf \color{red}0}&       25 \\
     Lang-10 &          &          &      \ding{109} &        &           &      &       &     &        &        \ding{109} &          &       &            &       &       {\bf \color{red}0}&       64 \\
     Lang-16 &          &          &      \ding{108} &        &           &      &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&       27 \\
     Lang-21 &          &        \ding{108} &        &        &           &      &     \ding{108} &     &        &          &          &       &            &       &       {\bf \color{red}0}&        2 \\
     Lang-24 &          &        \ding{108} &        &        &           &    \ding{109} &       &   \ding{108} &      \ding{108} &          &          &       &            &       &       {\bf \color{red}0}&       64 \\
     Lang-26 &          &          &        &      \ding{108} &           &      &       &     &      \ding{108} &          &          &       &            &       &       {\bf \color{red}0}&      112 \\
     Lang-27 &          &          &      \ding{108} &        &           &      &     \ding{109} &     &        &          &          &       &          \ding{109} &       &       {\bf \color{red}0}&       56 \\
     Lang-29 &          &        \ding{108} &        &        &           &      &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
     Lang-33 &          &          &      \ding{108} &        &           &    \ding{108} &     \ding{108} &     &      \ding{108} &          &          &       &            &       &       {\bf \color{red}0}&        7 \\
     Lang-35 &          &          &        &        &           &      &       &   \ding{108} &        &          &          &       &            &       &       {\bf \color{red}0}&        2 \\
     Lang-38 &          &          &        &        &           &  (\ding{108}) &       &     &      \ding{108} &          &          &       &            &       &       {\bf \color{red}0}&        3 \\
     Lang-39 &          &          &      \ding{108} &        &           &    \ding{109} &     \ding{109} &   \ding{109} &      \ding{109} &          &          &       &            &     \ding{109} &       {\bf \color{red}0}&       27 \\
     Lang-51 &          &        \ding{108} &        &        &         \ding{109} &  (\ding{108}) &     \ding{109} &     &      \ding{109} &        \ding{108} &          &       &            &     \ding{109} &       {\bf \color{red}0}&       {\bf \color{red}0}\\
\hline
      Math-1 &          &          &      \ding{109} &        &           &      &       &     &        &          &          &       &            &       &       {\bf \color{red}0}&       14 \\
     Math-20 &          &          &      \ding{109} &        &           &      &     \ding{109} &     &      \ding{109} &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
     Math-25 &          &          &        &        &           &      &       &   \ding{108} &        &          &          &       &            &       &       {\bf \color{red}0}&       {\bf \color{red}0}\\
     Math-35 &          &          &      \ding{108} &        &           &      &       &   \ding{108} &        &          &          &       &            &       &       {\bf \color{red}0}&        5 \\
     Math-61 &          &          &        &        &           &      &       &   \ding{108} &        &          &          &       &            &       &       {\bf \color{red}0}&        1 \\
    Math-104 &          &          &        &        &           &      &       &     &      \ding{109} &          &          &       &            &     \ding{109} &       {\bf \color{red}0}&       {\bf \color{red}0}\\
\hline
     Time-11 &          &          &        &        &           &      &     \ding{109} &     &      \ding{109} &          &        \ding{109} &     \ding{109} &          \ding{109} &     \ding{109} &       {\bf \color{red}0}&       {\bf \color{red}0}\\


\hline
\end{tabular}

